Performance Analysis of a Foreground Segmentation Neural Network Model

In recent years the interest in segmentation has been growing, being used in a wide range of applications such as fraud detection, anomaly detection in public health and intrusion detection. We present an ablation study of FgSegNet_v2, analysing its three stages: (i) Encoder, (ii) Feature Pooling Module and (iii) Decoder. The result of this study is a proposal of a variation of the aforementioned method that surpasses state of the art results. Three datasets are used for testing: CDNet2014, SBI2015 and CityScapes. In CDNet2014 we got an overall improvement compared to the state of the art, mainly in the LowFrameRate subset. The presented approach is promising as it produces comparable results with the state of the art (SBI2015 and Cityscapes datasets) in very different conditions, such as different lighting conditions.

==> review.tex <==
Comments to improve:

1)
-> More solid motivations and experiments to justify contributions

2)
-> More motivation on why we are doing this 
-> Guidelines on what drove us to do the experiments in that order
-> Results on table 6 are not convincing

3)
-> Add more comments / discussions in the final results and comparison sections (4.5)

4)
-> Optimization only done in one dataset ( ????? )
-> Results on CDNet2014 are biased since the optimization was done here
-> No comparisons on CityScapes





Abstract and Introduction are adequate:  Yes (x4)
Needs more experimental results: No (x2) / Yes (x2)
Needs comparative evaluation: No (x3) / Yes 
Improve critical discussion ? (validation): Yes (x4)
Figures are adequate ? (in number and quality): Yes (x4)
Conclusions/Future Work are convincing?: No (x3) / Yes
References are up-to-date and appropriate? Yes (x4)
Paper formatting needs adjustment? No (x4)
Improve English? No (x3) / Yes
